How does the Combined Risk Affect the Performance of Unsupervised Domain Adaptation Approaches?

Unsupervised domain adaptation (UDA) aims to train a target classifier with labeled samples from the source domain and unlabeled samples from the target domain. Classical UDA learning bounds show that target risk is upper bounded by three terms: source risk, distribution discrepancy, and combined risk. Based on the assumption that the combined risk is a small fixed value, methods based on this bound train a target classifier by only minimizing estimators of the source risk and the distribution discrepancy. However, the combined risk may increase when minimizing both estimators, which makes the target risk uncontrollable. Hence the target classifier cannot achieve ideal performance if we fail to control the combined risk. To control the combined risk, the key challenge takes root in the unavailability of the labeled samples in the target domain. To address this key challenge, we propose a method named E-MixNet. E-MixNet employs enhanced mixup, a generic vicinal distribution, on the labeled source samples and pseudo-labeled target samples to calculate a proxy of the combined risk. Experiments show that the proxy can effectively curb the increase of the combined risk when minimizing the source risk and distribution discrepancy. Furthermore, we show that if the proxy of the combined risk is added into loss functions of four representative UDA methods, their performance is also improved.

==> v1_2_related_work.tex <==
\section{Related Work}
\textbf{Domain Adaptation Theory.} From a theoretical point of view, the domain adaptation problem was rigorously investigated for the first time by Ben-David et al. \shortcite{ben2007analysis,ben2010theory}. The authors of these papers proposed to make use of the $\mathcal{H}\Delta\mathcal{H}$-divergence as the distribution distance to measure the marginal distribution discrepancy between source and target domains. Yishay Mansour et al. \shortcite{yishay2009domain} extended the theoretical results by introducing a new distribution distance, discrepancy distance, that is
tailored to DA problems with arbitrary loss
functions. Utilizing the Wasserstein metric, Jian Shen et al. \shortcite{shen2018wasserstein} developed a different learning bound based on the Wasserstein metric. Recently,  Zhang et al. \shortcite{pmlr-v97-zhang19i} developed a new distribution distance, Margin Disparity Discrepancy, which is built on a scalar-valued margin disparity function
estimating the difference of multi-class scoring hypotheses. The above works mainly focus on developing different distribution distance. In our paper, a more general and more flexible distribution distance, Double Loss Disparity Discrepancy, is proposed. Especially, the Margin Disparity Discrepancy is a special case of our distribution distance.

\textbf{Domain Adaptation Methods.} Here we mainly introduce domain-invariant features methods based on deep neural networks. DAN \cite{long2015learning} employed the multi-kernel MMD to align the feature of 6-8 layers in Alexnet. WDGRL \cite{shen2018wasserstein} employed the Wasserstein metric to learn an invariant representation in deep neural networks. DANN \cite{ganin2016domain} employed a domain discriminator to recognize which domain samples come from and deceived the domain discriminator by changing features so that an invariant representation can be learned during the adversarial procession. Furthermore, CDAN utilized the tensor product between feature and classifier prediction to grasp the multimodal information and an entropy condition to control the uncertainty of the classifier. Recently, Kumagai et al. \shortcite{kumagai2019unsupervised} utilized unilateral transformations to match distributions based on Maximum Mean Discrepancy \cite{baktashmotlagh2013unsupervised}. Wen et al. \shortcite{wen2019exploiting} proposed that jointly aligning holistic and local feature statistics can learn better domain-invariant features. HoMM \cite{chen2020Homm} pointed that matching lower-order rank moment is not enough to align distributions and proposed a higher-order rank moment matching method.
% To preserve the inherent structure of data, Yang et al. \shortcite{yang2020bi} proposed a Bi-Directional Generation domain adaptation model with consistent classifiers interpolating two intermediate domains to bridge source and target domains.

==> v1_5_experiments.tex <==
\section{Experiments}
% \begin{table*}[htbp]
% \caption{Results on Office-31 and Image-CLEF}
% \label{tab:of31}
% \vspace{-0.8em}
% \centering
% \begin{tabular}{l|ccccccc} \hline
% Method & A$\rightarrow$W &D$\rightarrow$W &W$\rightarrow$D &A$\rightarrow$D &D$\rightarrow$A &W$\rightarrow$A &Avg \\ \hline
% ResNet-50\cite{he2016deep}            &68.4$\pm$0.2 &96.7$\pm$0.1 &99.3$\pm$0.1 &68.9$\pm$0.2 &62.5$\pm$0.3 &60.7$\pm$0.3 &76.1\\
% DAN\cite{long2015learning} 		    &80.5$\pm$0.4 &97.1$\pm$0.2 &99.6$\pm$0.1 &78.6$\pm$0.2 &63.6$\pm$0.3 &62.8$\pm$0.2 &80.4\\
% RTN\cite{long2016unsupervised} 	    &84.5$\pm$0.2 &96.8$\pm$0.1 &99.4$\pm$0.1 &77.5$\pm$0.3 &66.2$\pm$0.2 &64.8$\pm$0.3 &81.6\\
% DANN\cite{ganin2016domain} 		    &82.0$\pm$0.4 &96.9$\pm$0.2 &99.1$\pm$0.1 &79.7$\pm$0.4 &68.2$\pm$0.4 &67.4$\pm$0.5 &82.2\\
% ADDA\cite{tzeng2017adversarial} 	    &86.2$\pm$0.5 &96.2$\pm$0.3 &98.4$\pm$0.3 &77.8$\pm$0.3 &69.5$\pm$0.4 &68.9$\pm$0.5 &82.9\\
% JAN\cite{long2013transfer} 		    &86.0$\pm$0.4 &96.7$\pm$0.3 &99.7$\pm$0.1 &85.1$\pm$0.4 &69.2$\pm$0.3 &70.7$\pm$0.5 &84.6\\
% MADA\cite{pei2018multi} 	    	    &90.0$\pm$0.1 &97.4$\pm$0.1 &99.6$\pm$0.1 &87.8$\pm$0.2 &70.3$\pm$0.3 &66.4$\pm$0.3 &85.2\\
% SimNet\cite{pinheiro2018unsupervised} &88.6$\pm$0.5 &98.2$\pm$0.2 &99.7$\pm$0.2 &85.3$\pm$0.3 &73.4$\pm$0.8 &71.8$\pm$0.6 &86.2\\
% MCD\cite{saito2018maximum} 		    &89.6$\pm$0.2 &98.5$\pm$0.1 &100.0$\pm$.0 &91.3$\pm$0.2 &69.6$\pm$0.1 &70.8$\pm$0.3 &86.6\\
% CDAN+E\cite{long2018conditional} 		&94.1$\pm$0.1 &98.6$\pm$0.1 &100.0$\pm$.0 &92.9$\pm$0.2 &71.0$\pm$0.3 &69.3$\pm$0.3 &87.7\\
% SymNets\cite{zhang2019domain}         &90.8$\pm$0.1 &98.8$\pm$0.3 &100.0$\pm$.0 &93.9$\pm$0.5 &74.6$\pm$0.6 &72.5$\pm$0.5 &88.4\\
% MDD\cite{pmlr-v97-zhang19i} 		    &94.5$\pm$0.3 &98.4$\pm$0.1 &100.0$\pm$.0 &93.5$\pm$0.2 &74.6$\pm$0.3 &72.2$\pm$0.1 &88.9\\
% {E-MixNet}                            &93.0 &99.0 &100.0 &95.6 &78.9 &74.7 &90.2 \\ 
% \hline
% \hline
% % \end{tabular}
% % \end{table*}

% % \begin{table*}[htbp]
% % \caption{Results on Image-CLEF}
% % \label{tab:image}
% % \vspace{0.5em}
% % \centering
% % \begin{tabular}{l|ccccccc} \hline
% Method & I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg \\ \hline
% ResNet-50\cite{he2016deep}        &74.8$\pm$0.3 &83.9$\pm$0.1 &91.5$\pm$0.3 &78.0$\pm$0.2 &65.5$\pm$0.3 &91.2$\pm$0.3 &80.7\\
% DAN\cite{long2015learning}  		&74.5$\pm$0.4 &82.2$\pm$0.2 &92.8$\pm$0.2 &86.3$\pm$0.4 &69.2$\pm$0.4 &89.8$\pm$0.4 &82.5\\
% DANN\cite{ganin2016domain} 		&75.0$\pm$0.6 &86.0$\pm$0.3 &96.2$\pm$0.4 &87.0$\pm$0.5 &74.3$\pm$0.5 &91.5$\pm$0.6 &85.0\\
% JAN\cite{long2013transfer} 		&76.8$\pm$0.4 &88.0$\pm$0.2 &94.7$\pm$0.2 &89.5$\pm$0.3 &74.2$\pm$0.3 &91.7$\pm$0.3 &85.8\\
% MADA\cite{pei2018multi} 		    &75.0$\pm$0.3 &87.9$\pm$0.2 &96.0$\pm$0.3 &88.8$\pm$0.3 &75.2$\pm$0.2 &92.2$\pm$0.3 &85.8\\
% CDAN+E\cite{long2018conditional} 	&77.7$\pm$0.3 &90.7$\pm$0.2 &97.7$\pm$0.3 &91.3$\pm$0.3 &74.2$\pm$0.2 &94.3$\pm$0.3 &87.7\\
% SymNets\cite{zhang2019domain}     &80.2$\pm$0.3 &93.6$\pm$0.2 &97.0$\pm$0.3 &93.4$\pm$0.3 &78.7$\pm$0.3 &96.4$\pm$0.1 &89.9\\
% E-MixNet  	                    &79.4 &95.0 &97.8 &94.8 &81.4 &96.5  &90.8\\
% \hline
% \end{tabular}
% % \vspace{-0.25cm}
% \end{table*}


\begin{table*}[ht]
\centering
\caption{Results on Office-Home (ResNet-50)}
\vspace{-0.8em}
\label{tab:OfHome}
\begin{tabular}{l|p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}} \hline
Method &A$\rightarrow$C &A$\rightarrow$P &A$\rightarrow$R &C$\rightarrow$A &C$\rightarrow$P &C$\rightarrow$R &P$\rightarrow$A &P$\rightarrow$C &P$\rightarrow$R &R$\rightarrow$A &R$\rightarrow$C &R$\rightarrow$P &Avg\\ \hline
ResNet-50 \cite{he2016deep}          &~34.9 &~50.0 &~58.0 &~37.4 &~41.9 &~46.2 &~38.5 &~31.2 &~60.4 &~53.9 &~41.2 &~59.9 &46.1\\
% DAN\cite{long2015learning}  		&~43.6 &~57.0 &~67.9 &~45.8 &~56.5 &~60.4 &~44.0 &~43.6 &~67.7 &~63.1 &~51.5 &~74.3 &56.3\\
DAN \cite{long2015learning}  		&~54.0 &~68.6 &~75.9 &~56.4 &~66.0 &~67.9 &~57.1 &~50.3 &~74.7 &~68.8 &~55.8 &~80.6 &64.7\\
% DANN\cite{ganin2016domain}		&~45.6 &~59.3 &~70.1 &~47.0 &~58.5 &~60.9 &~46.1 &~43.7 &~68.5 &~63.2 &~51.8 &~76.8 &57.6\\
DANN \cite{ganin2016domain}		    &~44.1 &~66.5 &~74.6 &~57.9 &~62.0 &~67.2 &~55.7 &~40.9 &~73.5 &~67.5 &~47.9 &~77.7 &61.3\\
JAN \cite{long2013transfer} 		    &~45.9 &~61.2 &~68.9 &~50.4 &~59.7 &~61.0 &~45.8 &~43.4 &~70.3 &~63.9 &~52.4 &~76.8 &58.3\\
% CDAN+E\cite{long2018conditional} 	&~50.7 &~70.6 &~76.0 &~57.6 &~70.0 &~70.0 &~57.4 &~50.9 &~77.3 &~70.9 &~56.7 &~81.6 &65.8\\
CDAN+E \cite{long2018conditional} 	&~47.0 &~69.4 &~75.8 &~61.0 &~68.8 &~70.8 &~60.2 &~47.1 &~77.9 &~70.8 &~51.4 &~81.7 &65.2\\
% SymNets\cite{zhang2019domain}  	&~47.7 &~72.9 &~78.5 &~64.2 &~71.3 &~74.2 &~64.2 &~48.8 &~79.5 &~74.5 &~52.6 &~82.7 &67.6\\
SymNets \cite{zhang2019domain}  	    &~46.0 &~73.8 &~78.2 &~\textbf{64.1} &~69.7 &~74.2 &~63.2 &~48.9 &~\textbf{80.0} &~\textbf{74.0} &~51.6 &~82.9 &67.2\\
MDD \cite{pmlr-v97-zhang19i}  		&~54.9 &~73.7 &~77.8 &~60.0 &~71.4 &~71.8 &~61.2 &~53.6 &~78.1 &~72.5 &~60.2 &~82.3 &68.1\\
{E-MixNet}                          &~\textbf{57.7} &~\textbf{76.6} &~\textbf{79.8} &~63.6 &~\textbf{74.1} &~\textbf{75.0} &~\textbf{63.4} &~\textbf{56.4} &~79.7 &~72.8 &~\textbf{62.4} &~\textbf{85.5} &\textbf{70.6} \\ 
\hline
% \hline
\end{tabular}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{The results of combination experiments on Office-Home (ResNet-50)}
\vspace{-0.8em}
\label{tab:OfHome_lbd}
\begin{tabular}{l|p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}} \hline
Method &A$\rightarrow$C &A$\rightarrow$P &A$\rightarrow$R &C$\rightarrow$A &C$\rightarrow$P &C$\rightarrow$R &P$\rightarrow$A &P$\rightarrow$C &P$\rightarrow$R &R$\rightarrow$A &R$\rightarrow$C &R$\rightarrow$P &Avg\\ \hline
DAN \cite{long2015learning}                     &~54.0 &~68.6 &~75.9 &~56.4 &~66.0 &~67.9 &~57.1 &~50.3 &~74.7 &~68.8 &~55.8 &~80.6 &64.7 \\
DAN+$\widetilde{\Lambda}^{\ell_{mse}}$          &~\textbf{57.0} &~\textbf{71.0} &~\textbf{77.9} &~\textbf{59.9} &~\textbf{72.6} &~\textbf{70.1} &~\textbf{58.1} &~\textbf{57.1} &~\textbf{77.3} &~\textbf{72.7} &~\textbf{64.7} &~\textbf{84.6} &\textbf{68.6} \\\hline
DANN \cite{ganin2016domain}                     &~44.1 &~66.5 &~74.6 &~57.9 &~62.0 &~67.2 &~55.7 &~40.9 &~73.5 &~67.5 &~47.9 &~77.7 &61.3 \\
DANN+$\widetilde{\Lambda}^{\ell_{mse}}$         &~\textbf{50.9} &~\textbf{69.6} &~\textbf{77.8} &~\textbf{61.9} &~\textbf{70.7} &~\textbf{71.6} &~\textbf{60.0} &~\textbf{49.5} &~\textbf{78.4} &~\textbf{71.8} &~\textbf{55.7} &~\textbf{83.7} &\textbf{66.8}\\ \hline
CDAN+E \cite{long2018conditional}               &~47.0 &~69.4 &~75.8 &~61.0 &~68.8 &~70.8 &~60.2 &~47.1 &~77.9 &~70.8 &~51.4 &~81.7 &65.2 \\ 
CDAN+E+$\widetilde{\Lambda}^{\ell_{mse}}$       &~\textbf{49.5} &~\textbf{70.1} &~\textbf{77.8} &~\textbf{64.3} &~\textbf{71.3} &~\textbf{74.2} &~\textbf{61.6} &~\textbf{50.6} &~\textbf{80.0} &~\textbf{73.5} &~\textbf{56.6} &~\textbf{84.1} &\textbf{67.8}\\ \hline
SymNets \cite{zhang2019domain}                  &~46.0 &~73.8 &~78.2 &~64.1 &~69.7 &~74.2 &~63.2 &~\textbf{48.9} &~80.0 &~74.0 &~51.6 &~82.9 &67.2\\
SymNets+$\widetilde{\Lambda}^{\ell_{mse}}$      &~\textbf{48.8} &~\textbf{74.7} &~\textbf{79.7} &~\textbf{64.9} &~\textbf{72.5} &~\textbf{75.6} &~\textbf{63.9} &~47.0 &~\textbf{80.8} &~\textbf{73.9} &~\textbf{52.4} &~\textbf{83.9} &\textbf{68.2} \\ 
%MDD\cite{pmlr-v97-zhang19i} &54.1 &73.0 &77.4 &59.0 &69.&70.8 &58.5 &52.2 &77.2 &70.0 &56.4 &82.6 &66.8 \\
%MDD+$\tilde{\lambda}$ &57.7 &76.6 &79.8 &63.6 &74.1 &75.&63.4 &56.4 &79.7 &72.8 &62.4 &85.5 &70.6 \\ 
\hline
\end{tabular}
% \vspace{-4.5em}
\end{table*}

% \begin{table*}[htbp]
% \caption{Ablation experiments on Image-CLEF}
% \label{tab:aba}
% \vspace{-0.8em}
% \centering
% \begin{tabular}{cccc|ccccccc} \hline
% source &target &mixup &emixup &I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg\\ \hline
% &&& &80.2 &94.2 &96.7 &94.7 &79.2 &95.5 &90.1\\
% &$\surd$&& &&&&&&&\\
% &$\surd$&$\surd$& &79.7 &93.7 &97.5 &94.5 &79.7 &96.2 &90.2\\
% $\surd$&$\surd$&$\surd$& &79.4 &95.0 &97.8 &94.8 &81.4 &96.5 &90.8\\
% $\surd$&$\surd$&$\surd$&$\surd$ &80.5 &96.0 &97.7 &95.2 &79.9 &97.0 &91.0\\	\hline
% \end{tabular}
% % \vspace{-0.5em}
% \end{table*}

\begin{table}[htbp]
\caption{Ablation experiments on Image-CLEF}
\label{tab:aba}
\vspace{-0.8em}
\centering
%\begin{tabular}{cccc|ccccccc} \hline
\begin{tabular}{p{0.08cm}p{0.08cm}p{0.08cm}p{0.08cm}|p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}} \hline
s &t &m &e
%source &target &mixup &emixup
&I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg\\ \hline
&&&                                                 &80.2 &94.2 &96.7 &94.7 &79.2 &95.5 &90.1\\
&$\small{\surd}$&&                                  &79.9 &92.2 &97.7 &93.8 &79.4 &96.5 &89.9\\
&$\small{\surd}$&$\small{\surd}$&                   &79.7 &93.7 &97.5 &94.5 &79.7 &96.2 &90.2\\
$\small{\surd}$&$\small{\surd}$&$\small{\surd}$&    &79.4 &95.0 &\textbf{97.8} &94.8 &\textbf{81.4} &96.5 &90.8\\
$\small{\surd}$&$\small{\surd}$& &$\small{\surd}$   &\textbf{80.5} &\textbf{96.0} &97.7 &\textbf{95.2} &79.9 &\textbf{97.0} &\textbf{91.0}\\	\hline
\end{tabular}
% \vspace{-0.5em}
\end{table}

We evaluate E-Mixnet on three public datasets, and compare it with several existing state-of-the-art methods. %Furthermore, we further test the efficacy of the proxy of the combined risk by adding it into the loss function of four representative UDA methods.

\subsection{Datasets}
Three common UDA datasets are used to evaluate the efficacy of E-MixNet. 

\textbf{Office-31} \cite{saenko2010adapting} is an object recognition dataset with $4,110$ images, which consists of three domains with a slight discrepancy: \textit{amazon} ({A}), \textit{dslr} ({D}) and \textit{webcam} ({W}). Each domain contains $31$ kinds of objects. So there are $6$ domain adaptation tasks on \textit{Office-31}: {A} $\rightarrow$ {D}, {A} $\rightarrow$ {W}, {D} $\rightarrow$ {A}, {D} $\rightarrow$ {W}, {W} $\rightarrow$ {A}, {W} $\rightarrow$ {D}. 

\textbf{Office-Home} \cite{venkateswara2017deep} is an object recognition dataset with $15,500$ image, which contains four domains with more obvious domain discrepancy than \textit{Office-31}. These domains are \textit{Artistic} ({A}), \textit{Clipart} ({C}), \textit{Product} ({P}), \textit{Real-World} ({R}). Each domain contains $65$ kinds of objects. So there are $12$ domain adaptation tasks on {Office-Home}: {A} $\rightarrow$ {C}, {A} $\rightarrow$ {P}, {A} $\rightarrow$ {R}, ..., {R} $\rightarrow$ {P}. 

\textbf{ImageCLEF-DA}\footnote{http://imageclef.org/2014/adaptation/} is a dataset organized by selecting the 12 common classes shared by three public datasets (domains): \textit{Caltech-256} (C), \textit{ImageNet ILSVRC} 2012 (I), and \textit{Pascal VOC} 2012 (P). We permute all three domains and build six transfer tasks: I$\rightarrow$P, P$\rightarrow$I, I$\rightarrow$C, C$\rightarrow$I, C$\rightarrow$P, P$\rightarrow$C.

\subsection{Experimental Setup}
Following the standard protocol for unsupervised domain adaptation in \cite{ganin2016domain, long2018conditional}, all labeled source  samples and unlabeled target samples are used in the training process and we report the average classification accuracy based on three random experiments. $\gamma$ in Eq. \eqref{eq:loss_dd} is selected from {2, 4, 8}, and it is set to 2 for Office-Home, 4 for Office-31, and 8 for Image-CLEF.

ResNet-50 \cite{he2016deep} pretrained on ImageNet is employed as the backbone network ($\mathbf{G}$). $\mathbf{C}$, $\mathbf{D}$ and $\mathbf{C}^*$ are all two fully connected layers where the hidden unit is 1024. Gradient reversal layer between \textbf{G} and $\mathbf{D}$ is employed for adversarial training. The algorithm is implemented by Pytorch. The mini-batch stochastic gradient descent with momentum 0.9 is employed as the optimizer, and the learning rate is adjected by $l_i = l_0(1+\delta i)^{-\beta}$, where i linearly increase from 0 to 1 during the training process, $\delta=10$, $l_0=0.04$. We follow \cite{pmlr-v97-zhang19i} to employ a progressive strategy for $\eta$: $\eta=\frac{2\eta_0}{1+\exp(\delta*i)-\eta_0}$, $\eta_0$ is set to 0.1. The $\alpha$ in e-mixup is set to 0.6 in all experiments.

\subsection{Results}
\vspace{-0.125em}
The results on \textit{Office-31} are reported in Tabel \ref{tab:of31}. E-MixNet achieves the best results and exceeds the baselines for 4 of 6 tasks. Compared to the competitive baseline MDD, E-MixNet surpasses it by 4.3\% for the difficult task D $\rightarrow$ A.

The results on \textit{Image-CLEF} are reported in Table \ref{tab:image}. E-MixNet significantly outperforms the baselines for 5 of 6 tasks. For the hard task C $\rightarrow$ P, E-MixNet surpasses the competitive baseline SymNets by 2.7\%.

The results on \textit{Office-Home} are reported in Table \ref{tab:OfHome}. Despite \textit{Office-Home} is a challenging dataset, E-MixNet still achieves better performance than all the baselines for 9 of 12 tasks. For the difficult tasks A $\rightarrow$ C, P $\rightarrow$ A, and R $\rightarrow$ C, E-MixNet has significant advantages.

In order to further verify the efficacy of the proposed proxy of the combined risk, we add the proxy into the loss functions of four representative UDA methods, which are DAN, DANN, CDAN, and SymNets. As shown in Fig. \ref{fig:network}(a), we add a new classifier that is the same as the classifier in the original method to formulate the proxy of the combined risk. The results are shown in Table \ref{tab:OfHome_lbd}. The four methods can achieve better performance after optimizing the proxy. It is worth noting that DANN obtains a $5$  percent increase. The experiments adequately demonstrate the combined risk plays a crucial role for methods that aim to learn a domain-invariant representation  and the proxy can indeed curb the increase of the combined risk.

\subsection{Ablation Study and Parameter Analysis}
\textit{Ablation Study}. To further verify the efficacy of the proxy of combined risk calculated by mixup and e-mixup respectively. Ablation experiments are shown in Tabel \ref{tab:aba}, where s indicates that the source samples are introduced to augment the target samples, t indicates augmenting the target samples, m denotes mixup, and e denotes e-mixup. Table \ref{tab:aba} shows that E-MixNet achieves the best performance, which further shows that we can effectively control the combined risk by the proxy $\widetilde{\Lambda}^{{\ell}_{mse}}$.

\noindent \textit{Parameter analysis}. 
% E-MixNet will degrade to MDD \cite{pmlr-v97-zhang19i}, when the proxy of combined risk is ignored.
% When we set $\ell_s$ and $\ell_t$ as cross-entropy and modified cross-entropy \cite{pmlr-v97-zhang19i, NIPS2014_5423}, the double loss disparity discrepancy will become a substitute of Margin Disparity Discrepancy \cite{pmlr-v97-zhang19i}.
% In MDD, the parameter $\gamma$ in Eq. \eqref{eq:loss_dd} is related to the \textit{margin}. 
Here we aim to study how the parameter $\gamma$ affects the performance and the efficiencies of \emph{mean square error} (MSE) and cross-entropy for the proxy of combined risk. Firstly, as shown in Fig. \ref{fig:param}(a), a relatively larger $\gamma$ can obtain better performance and faster convergence. Secondly, when \textit{mixup} behaves between two samples, the accuracy of the pseudo labels of the target samples are much important. To against the adversarial samples, MSE is employed to substitute cross-entropy. As shown in Fig. \ref{fig:param}(b), compared to cross-entropy, MSE can obtain more stable
and better performance. Due to the limited space, the analysis of $\alpha$ and visualizations are shown in Appendix.

\begin{figure}[!t]
\centering
\includegraphics[scale=0.3,trim=5 16 0 0, clip]{param_3.pdf}
\caption{The test accuracy on C $\rightarrow$ P. 
    The impact of $\gamma$ is shown in (a). The impact of the loss functions for the proxy of the combined risk is shown in (b). 
    % The impact of $\alpha$ is shown in (c).
    }
\label{fig:param}
\vspace{-1.5em}
\end{figure}

% \begin{figure}[!t]
% \centering
% \label{fig:param}
% \subfigure[]{
%     \begin{minipage}[t]{0.65\linewidth}
%         \centering
%         \includegraphics[width=1.651in]{param_3.pdf}\\
%         \vspace{0.02cm}
%     \end{minipage}%
% }
% \subfigure[]{
%     \begin{minipage}[t]{0.33\linewidth}
%         \centering
%         \includegraphics[width=1.651in]{ADistance.pdf}\\
%         \vspace{0.02cm}
%         %\caption{fig1}
%     \end{minipage}%
% }
% \vspace{-1.5em}
% \end{figure}

% Furthermore, parameter $\alpha$ also plays a crucial role in the proxy of combined risk. It is different from the usage of \textit{mixup} in \cite{zhang2018mixup, berthelot2019mixmatch}, for simplicity, we set $\alpha$ as the fixed value in all the experiments. As shown in Fig. \ref{fig:param}(c), better performance can be achieved when $\alpha$ is set to 0.6. In addition, selecting $\alpha$ in [0.4, 0.6] is recommended.
%1: gamma; 2:alpha; 3:mse and cross-entropy; 4.E-mixup and mixup;


==> v3_5_experiments.tex <==
\section{Experiments}
% \begin{table*}[htbp]
% \caption{Results on Office-31 and Image-CLEF}
% \label{tab:of31}
% \vspace{-0.8em}
% \centering
% \begin{tabular}{l|ccccccc} \hline
% Method & A$\rightarrow$W &D$\rightarrow$W &W$\rightarrow$D &A$\rightarrow$D &D$\rightarrow$A &W$\rightarrow$A &Avg \\ \hline
% ResNet-50\cite{he2016deep}            &68.4$\pm$0.2 &96.7$\pm$0.1 &99.3$\pm$0.1 &68.9$\pm$0.2 &62.5$\pm$0.3 &60.7$\pm$0.3 &76.1\\
% DAN\cite{long2015learning} 		    &80.5$\pm$0.4 &97.1$\pm$0.2 &99.6$\pm$0.1 &78.6$\pm$0.2 &63.6$\pm$0.3 &62.8$\pm$0.2 &80.4\\
% RTN\cite{long2016unsupervised} 	    &84.5$\pm$0.2 &96.8$\pm$0.1 &99.4$\pm$0.1 &77.5$\pm$0.3 &66.2$\pm$0.2 &64.8$\pm$0.3 &81.6\\
% DANN\cite{ganin2016domain} 		    &82.0$\pm$0.4 &96.9$\pm$0.2 &99.1$\pm$0.1 &79.7$\pm$0.4 &68.2$\pm$0.4 &67.4$\pm$0.5 &82.2\\
% ADDA\cite{tzeng2017adversarial} 	    &86.2$\pm$0.5 &96.2$\pm$0.3 &98.4$\pm$0.3 &77.8$\pm$0.3 &69.5$\pm$0.4 &68.9$\pm$0.5 &82.9\\
% JAN\cite{long2013transfer} 		    &86.0$\pm$0.4 &96.7$\pm$0.3 &99.7$\pm$0.1 &85.1$\pm$0.4 &69.2$\pm$0.3 &70.7$\pm$0.5 &84.6\\
% MADA\cite{pei2018multi} 	    	    &90.0$\pm$0.1 &97.4$\pm$0.1 &99.6$\pm$0.1 &87.8$\pm$0.2 &70.3$\pm$0.3 &66.4$\pm$0.3 &85.2\\
% SimNet\cite{pinheiro2018unsupervised} &88.6$\pm$0.5 &98.2$\pm$0.2 &99.7$\pm$0.2 &85.3$\pm$0.3 &73.4$\pm$0.8 &71.8$\pm$0.6 &86.2\\
% MCD\cite{saito2018maximum} 		    &89.6$\pm$0.2 &98.5$\pm$0.1 &100.0$\pm$.0 &91.3$\pm$0.2 &69.6$\pm$0.1 &70.8$\pm$0.3 &86.6\\
% CDAN+E\cite{long2018conditional} 		&94.1$\pm$0.1 &98.6$\pm$0.1 &100.0$\pm$.0 &92.9$\pm$0.2 &71.0$\pm$0.3 &69.3$\pm$0.3 &87.7\\
% SymNets\cite{zhang2019domain}         &90.8$\pm$0.1 &98.8$\pm$0.3 &100.0$\pm$.0 &93.9$\pm$0.5 &74.6$\pm$0.6 &72.5$\pm$0.5 &88.4\\
% MDD\cite{pmlr-v97-zhang19i} 		    &94.5$\pm$0.3 &98.4$\pm$0.1 &100.0$\pm$.0 &93.5$\pm$0.2 &74.6$\pm$0.3 &72.2$\pm$0.1 &88.9\\
% {E-MixNet}                            &93.0 &99.0 &100.0 &95.6 &78.9 &74.7 &90.2 \\ 
% \hline
% \hline
% % \end{tabular}
% % \end{table*}

% % \begin{table*}[htbp]
% % \caption{Results on Image-CLEF}
% % \label{tab:image}
% % \vspace{0.5em}
% % \centering
% % \begin{tabular}{l|ccccccc} \hline
% Method & I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg \\ \hline
% ResNet-50\cite{he2016deep}        &74.8$\pm$0.3 &83.9$\pm$0.1 &91.5$\pm$0.3 &78.0$\pm$0.2 &65.5$\pm$0.3 &91.2$\pm$0.3 &80.7\\
% DAN\cite{long2015learning}  		&74.5$\pm$0.4 &82.2$\pm$0.2 &92.8$\pm$0.2 &86.3$\pm$0.4 &69.2$\pm$0.4 &89.8$\pm$0.4 &82.5\\
% DANN\cite{ganin2016domain} 		&75.0$\pm$0.6 &86.0$\pm$0.3 &96.2$\pm$0.4 &87.0$\pm$0.5 &74.3$\pm$0.5 &91.5$\pm$0.6 &85.0\\
% JAN\cite{long2013transfer} 		&76.8$\pm$0.4 &88.0$\pm$0.2 &94.7$\pm$0.2 &89.5$\pm$0.3 &74.2$\pm$0.3 &91.7$\pm$0.3 &85.8\\
% MADA\cite{pei2018multi} 		    &75.0$\pm$0.3 &87.9$\pm$0.2 &96.0$\pm$0.3 &88.8$\pm$0.3 &75.2$\pm$0.2 &92.2$\pm$0.3 &85.8\\
% CDAN+E\cite{long2018conditional} 	&77.7$\pm$0.3 &90.7$\pm$0.2 &97.7$\pm$0.3 &91.3$\pm$0.3 &74.2$\pm$0.2 &94.3$\pm$0.3 &87.7\\
% SymNets\cite{zhang2019domain}     &80.2$\pm$0.3 &93.6$\pm$0.2 &97.0$\pm$0.3 &93.4$\pm$0.3 &78.7$\pm$0.3 &96.4$\pm$0.1 &89.9\\
% E-MixNet  	                    &79.4 &95.0 &97.8 &94.8 &81.4 &96.5  &90.8\\
% \hline
% \end{tabular}
% % \vspace{-0.25cm}
% \end{table*}


\begin{table*}[ht]
\centering
\caption{Results on Office-Home (ResNet-50)}
\vspace{-0.8em}
\label{tab:OfHome}
\begin{tabular}{l|p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}} \hline
Method &A$\rightarrow$C &A$\rightarrow$P &A$\rightarrow$R &C$\rightarrow$A &C$\rightarrow$P &C$\rightarrow$R &P$\rightarrow$A &P$\rightarrow$C &P$\rightarrow$R &R$\rightarrow$A &R$\rightarrow$C &R$\rightarrow$P &Avg\\ \hline
ResNet-50 \cite{he2016deep}          &~34.9 &~50.0 &~58.0 &~37.4 &~41.9 &~46.2 &~38.5 &~31.2 &~60.4 &~53.9 &~41.2 &~59.9 &46.1\\
% DAN\cite{long2015learning}  		&~43.6 &~57.0 &~67.9 &~45.8 &~56.5 &~60.4 &~44.0 &~43.6 &~67.7 &~63.1 &~51.5 &~74.3 &56.3\\
DAN \cite{long2015learning}  		&~54.0 &~68.6 &~75.9 &~56.4 &~66.0 &~67.9 &~57.1 &~50.3 &~74.7 &~68.8 &~55.8 &~80.6 &64.7\\
% DANN\cite{ganin2016domain}		&~45.6 &~59.3 &~70.1 &~47.0 &~58.5 &~60.9 &~46.1 &~43.7 &~68.5 &~63.2 &~51.8 &~76.8 &57.6\\
DANN \cite{ganin2016domain}		    &~44.1 &~66.5 &~74.6 &~57.9 &~62.0 &~67.2 &~55.7 &~40.9 &~73.5 &~67.5 &~47.9 &~77.7 &61.3\\
JAN \cite{long2013transfer} 		    &~45.9 &~61.2 &~68.9 &~50.4 &~59.7 &~61.0 &~45.8 &~43.4 &~70.3 &~63.9 &~52.4 &~76.8 &58.3\\
% CDAN+E\cite{long2018conditional} 	&~50.7 &~70.6 &~76.0 &~57.6 &~70.0 &~70.0 &~57.4 &~50.9 &~77.3 &~70.9 &~56.7 &~81.6 &65.8\\
CDAN+E \cite{long2018conditional} 	&~47.0 &~69.4 &~75.8 &~61.0 &~68.8 &~70.8 &~60.2 &~47.1 &~77.9 &~70.8 &~51.4 &~81.7 &65.2\\
% SymNets\cite{zhang2019domain}  	&~47.7 &~72.9 &~78.5 &~64.2 &~71.3 &~74.2 &~64.2 &~48.8 &~79.5 &~74.5 &~52.6 &~82.7 &67.6\\
SymNets \cite{zhang2019domain}  	    &~46.0 &~73.8 &~78.2 &~\textbf{64.1} &~69.7 &~74.2 &~63.2 &~48.9 &~\textbf{80.0} &~\textbf{74.0} &~51.6 &~82.9 &67.2\\
MDD \cite{pmlr-v97-zhang19i}  		&~54.9 &~73.7 &~77.8 &~60.0 &~71.4 &~71.8 &~61.2 &~53.6 &~78.1 &~72.5 &~60.2 &~82.3 &68.1\\
{E-MixNet}                          &~\textbf{57.7} &~\textbf{76.6} &~\textbf{79.8} &~63.6 &~\textbf{74.1} &~\textbf{75.0} &~\textbf{63.4} &~\textbf{56.4} &~79.7 &~72.8 &~\textbf{62.4} &~\textbf{85.5} &\textbf{70.6} \\ 
\hline
% \hline
\end{tabular}
\vspace{-0.5em}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{The results of combination experiments on Office-Home (ResNet-50)}
\vspace{-1em}
\label{tab:OfHome_lbd}
\begin{tabular}{l|p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}} \hline
Method &A$\rightarrow$C &A$\rightarrow$P &A$\rightarrow$R &C$\rightarrow$A &C$\rightarrow$P &C$\rightarrow$R &P$\rightarrow$A &P$\rightarrow$C &P$\rightarrow$R &R$\rightarrow$A &R$\rightarrow$C &R$\rightarrow$P &Avg\\ \hline
DAN \cite{long2015learning}                     &~54.0 &~68.6 &~75.9 &~56.4 &~66.0 &~67.9 &~57.1 &~50.3 &~74.7 &~68.8 &~55.8 &~80.6 &64.7 \\
DAN+$\widetilde{\Lambda}^{\ell_{mse}}$          &~\textbf{57.0} &~\textbf{71.0} &~\textbf{77.9} &~\textbf{59.9} &~\textbf{72.6} &~\textbf{70.1} &~\textbf{58.1} &~\textbf{57.1} &~\textbf{77.3} &~\textbf{72.7} &~\textbf{64.7} &~\textbf{84.6} &\textbf{68.6} \\\hline
DANN \cite{ganin2016domain}                     &~44.1 &~66.5 &~74.6 &~57.9 &~62.0 &~67.2 &~55.7 &~40.9 &~73.5 &~67.5 &~47.9 &~77.7 &61.3 \\
DANN+$\widetilde{\Lambda}^{\ell_{mse}}$         &~\textbf{50.9} &~\textbf{69.6} &~\textbf{77.8} &~\textbf{61.9} &~\textbf{70.7} &~\textbf{71.6} &~\textbf{60.0} &~\textbf{49.5} &~\textbf{78.4} &~\textbf{71.8} &~\textbf{55.7} &~\textbf{83.7} &\textbf{66.8}\\ \hline
CDAN+E \cite{long2018conditional}               &~47.0 &~69.4 &~75.8 &~61.0 &~68.8 &~70.8 &~60.2 &~47.1 &~77.9 &~70.8 &~51.4 &~81.7 &65.2 \\ 
CDAN+E+$\widetilde{\Lambda}^{\ell_{mse}}$       &~\textbf{49.5} &~\textbf{70.1} &~\textbf{77.8} &~\textbf{64.3} &~\textbf{71.3} &~\textbf{74.2} &~\textbf{61.6} &~\textbf{50.6} &~\textbf{80.0} &~\textbf{73.5} &~\textbf{56.6} &~\textbf{84.1} &\textbf{67.8}\\ \hline
SymNets \cite{zhang2019domain}                  &~46.0 &~73.8 &~78.2 &~64.1 &~69.7 &~74.2 &~63.2 &~\textbf{48.9} &~80.0 &~74.0 &~51.6 &~82.9 &67.2\\
SymNets+$\widetilde{\Lambda}^{\ell_{mse}}$      &~\textbf{48.8} &~\textbf{74.7} &~\textbf{79.7} &~\textbf{64.9} &~\textbf{72.5} &~\textbf{75.6} &~\textbf{63.9} &~47.0 &~\textbf{80.8} &~\textbf{73.9} &~\textbf{52.4} &~\textbf{83.9} &\textbf{68.2} \\ 
%MDD\cite{pmlr-v97-zhang19i} &54.1 &73.0 &77.4 &59.0 &69.&70.8 &58.5 &52.2 &77.2 &70.0 &56.4 &82.6 &66.8 \\
%MDD+$\tilde{\lambda}$ &57.7 &76.6 &79.8 &63.6 &74.1 &75.&63.4 &56.4 &79.7 &72.8 &62.4 &85.5 &70.6 \\ 
\hline
\end{tabular}
\vspace{-1em}
\end{table*}

% \begin{table*}[htbp]
% \caption{Ablation experiments on Image-CLEF}
% \label{tab:aba}
% \vspace{-0.8em}
% \centering
% \begin{tabular}{cccc|ccccccc} \hline
% source &target &mixup &emixup &I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg\\ \hline
% &&& &80.2 &94.2 &96.7 &94.7 &79.2 &95.5 &90.1\\
% &$\surd$&& &&&&&&&\\
% &$\surd$&$\surd$& &79.7 &93.7 &97.5 &94.5 &79.7 &96.2 &90.2\\
% $\surd$&$\surd$&$\surd$& &79.4 &95.0 &97.8 &94.8 &81.4 &96.5 &90.8\\
% $\surd$&$\surd$&$\surd$&$\surd$ &80.5 &96.0 &97.7 &95.2 &79.9 &97.0 &91.0\\	\hline
% \end{tabular}
% % \vspace{-0.5em}
% \end{table*}

\begin{table}[htbp]
\caption{Ablation experiments on Image-CLEF}
\label{tab:aba}
\vspace{-0.8em}
\centering
%\begin{tabular}{cccc|ccccccc} \hline
\begin{tabular}{p{0.08cm}p{0.08cm}p{0.08cm}p{0.08cm}|p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}p{0.45cm}} \hline
s &t &m &e
%source &target &mixup &emixup
&I$\rightarrow$P &P$\rightarrow$I &I$\rightarrow$C &C$\rightarrow$I &C$\rightarrow$P &P$\rightarrow$C &Avg\\ \hline
&&&                                                 &80.2 &94.2 &96.7 &94.7 &79.2 &95.5 &90.1\\
&$\small{\surd}$&&                                  &79.9 &92.2 &97.7 &93.8 &79.4 &96.5 &89.9\\
&$\small{\surd}$&$\small{\surd}$&                   &79.7 &93.7 &97.5 &94.5 &79.7 &96.2 &90.2\\
$\small{\surd}$&$\small{\surd}$&$\small{\surd}$&    &79.4 &95.0 &\textbf{97.8} &94.8 &\textbf{81.4} &96.5 &90.8\\
$\small{\surd}$&$\small{\surd}$& &$\small{\surd}$   &\textbf{80.5} &\textbf{96.0} &97.7 &\textbf{95.2} &79.9 &\textbf{97.0} &\textbf{91.0}\\	\hline
\end{tabular}
\vspace{-1em}
\end{table}

We evaluate E-Mixnet on three public datasets, and compare it with several existing state-of-the-art methods. %Furthermore, we further test the efficacy of the proxy of the combined risk by adding it into the loss function of four representative UDA methods.

\subsection{Datasets}
Three common UDA datasets are used to evaluate the efficacy of E-MixNet. 

\textbf{Office-31} \cite{saenko2010adapting} is an object recognition dataset with $4,110$ images, which consists of three domains with a slight discrepancy: \textit{amazon} ({A}), \textit{dslr} ({D}) and \textit{webcam} ({W}). Each domain contains $31$ kinds of objects. So there are $6$ domain adaptation tasks on \textit{Office-31}: {A} $\rightarrow$ {D}, {A} $\rightarrow$ {W}, {D} $\rightarrow$ {A}, {D} $\rightarrow$ {W}, {W} $\rightarrow$ {A}, {W} $\rightarrow$ {D}. 

\textbf{Office-Home} \cite{venkateswara2017deep} is an object recognition dataset with $15,500$ image, which contains four domains with more obvious domain discrepancy than \textit{Office-31}. These domains are \textit{Artistic} ({A}), \textit{Clipart} ({C}), \textit{Product} ({P}), \textit{Real-World} ({R}). Each domain contains $65$ kinds of objects. So there are $12$ domain adaptation tasks on {Office-Home}: {A} $\rightarrow$ {C}, {A} $\rightarrow$ {P}, {A} $\rightarrow$ {R}, ..., {R} $\rightarrow$ {P}. 

\textbf{ImageCLEF-DA}\footnote{http://imageclef.org/2014/adaptation/} is a dataset organized by selecting the 12 common classes shared by three public datasets (domains): \textit{Caltech-256} (C), \textit{ImageNet ILSVRC} 2012 (I), and \textit{Pascal VOC} 2012 (P). We permute all three domains and build six transfer tasks: I$\rightarrow$P, P$\rightarrow$I, I$\rightarrow$C, C$\rightarrow$I, C$\rightarrow$P, P$\rightarrow$C.

\subsection{Experimental Setup}
Following the standard protocol for unsupervised domain adaptation in \cite{ganin2016domain, long2018conditional}, all labeled source  samples and unlabeled target samples are used in the training process and we report the average classification accuracy based on three random experiments. $\gamma$ in Eq. \eqref{eq:loss_dd} is selected from {2, 4, 8}, and it is set to 2 for Office-Home, 4 for Office-31, and 8 for Image-CLEF.

ResNet-50 \cite{he2016deep} pretrained on ImageNet is employed as the backbone network ($\mathbf{G}$). $\mathbf{C}$, $\mathbf{D}$ and $\mathbf{C}^*$ are all two fully connected layers where the hidden unit is 1024. Gradient reversal layer between \textbf{G} and $\mathbf{D}$ is employed for adversarial training. The algorithm is implemented by Pytorch. The mini-batch stochastic gradient descent with momentum 0.9 is employed as the optimizer, and the learning rate is adjected by $l_i = l_0(1+\delta i)^{-\beta}$, where i linearly increase from 0 to 1 during the training process, $\delta=10$, $l_0=0.04$. We follow \cite{pmlr-v97-zhang19i} to employ a progressive strategy for $\eta$: $\eta=\frac{2\eta_0}{1+\exp(\delta*i)-\eta_0}$, $\eta_0$ is set to 0.1. The $\alpha$ in e-mixup is set to 0.6 in all experiments.

\subsection{Results}
\vspace{-0.125em}
The results on \textit{Office-31} are reported in Tabel \ref{tab:of31}. E-MixNet achieves the best results and exceeds the baselines for 4 of 6 tasks. Compared to the competitive baseline MDD, E-MixNet surpasses it by 4.3\% for the difficult task D $\rightarrow$ A.

The results on \textit{Image-CLEF} are reported in Table \ref{tab:image}. E-MixNet significantly outperforms the baselines for 5 of 6 tasks. For the hard task C $\rightarrow$ P, E-MixNet surpasses the competitive baseline SymNets by 2.7\%.

The results on \textit{Office-Home} are reported in Table \ref{tab:OfHome}. Despite \textit{Office-Home} is a challenging dataset, E-MixNet still achieves better performance than all the baselines for 9 of 12 tasks. For the difficult tasks A $\rightarrow$ C, P $\rightarrow$ A, and R $\rightarrow$ C, E-MixNet has significant advantages.

In order to further verify the efficacy of the proposed proxy of the combined risk, we add the proxy into the loss functions of four representative UDA methods. As shown in Fig. \ref{fig:network}(a), we add a new classifier that is the same as the classifier in the original method to formulate the proxy of the combined risk. The results are shown in Table \ref{tab:OfHome_lbd}. The four methods can achieve better performance after optimizing the proxy. It is worth noting that DANN obtains a 5.5\% percent increase. The experiments adequately demonstrate the combined risk plays a crucial role for methods that aim to learn a domain-invariant representation and the proxy can indeed curb the increase of the combined risk.

\subsection{Ablation Study and Parameter Analysis}
\textit{Ablation Study}. To further verify the efficacy of the proxy of combined risk calculated by mixup and e-mixup respectively. Ablation experiments are shown in Tabel \ref{tab:aba}, where s indicates that the source samples are introduced to augment the target samples, t indicates augmenting the target samples, m denotes mixup, and e denotes e-mixup. Table \ref{tab:aba} shows that E-MixNet achieves the best performance, which further shows that we can effectively control the combined risk by the proxy $\widetilde{\Lambda}^{{\ell}_{mse}}$.

\noindent \textit{Parameter analysis}. 
% E-MixNet will degrade to MDD \cite{pmlr-v97-zhang19i}, when the proxy of combined risk is ignored.
% When we set $\ell_s$ and $\ell_t$ as cross-entropy and modified cross-entropy \cite{pmlr-v97-zhang19i, NIPS2014_5423}, the double loss disparity discrepancy will become a substitute of Margin Disparity Discrepancy \cite{pmlr-v97-zhang19i}.
% In MDD, the parameter $\gamma$ in Eq. \eqref{eq:loss_dd} is related to the \textit{margin}. 
Here we aim to study how the parameter $\gamma$ affects the performance and the efficiencies of \emph{mean square error} (MSE) and cross-entropy for the proxy of combined risk. Firstly, as shown in Fig. \ref{fig:param}(a), a relatively larger $\gamma$ can obtain better performance and faster convergence. Secondly, when \textit{mixup} behaves between two samples, the accuracy of the pseudo labels of the target samples are much important. To against the adversarial samples, MSE is employed to substitute cross-entropy. As shown in Fig. \ref{fig:param}(b), MSE can obtain more stable and better performance. 
% Due to the limited space, the analysis of $\alpha$ and visualizations are shown in Appendix. 
Furthermore, $\mathcal{A}$-distance is also an important indicator showing the distribution discrepancy, which is defined as $dis_{\mathcal{A}=2(1-2\epsilon)}$ where $\epsilon$ is the test error. As shown in Fig. \ref{fig:param} (c). E-MixNet achieves a better performance of adaptation, implying the efficiency of the proposed proxy.

\begin{figure}[!t]
\centering
\includegraphics[scale=0.3,trim=5 16 0 0, clip]{param_4.pdf}
\caption{The impact of $\gamma$ is shown in (a). The impact of the loss functions for the proxy of the combined risk is shown in (b). Comparison of $\mathcal{A}-distance.$
    % The impact of $\alpha$ is shown in (c).
    }
\label{fig:param}
\vspace{-1.5em}
\end{figure}

% \begin{figure}[!t]
% \centering
% \label{fig:param}
% \subfigure[]{
%     \begin{minipage}[t]{0.65\linewidth}
%         \centering
%         \includegraphics[width=1.651in]{param_3.pdf}\\
%         \vspace{0.02cm}
%     \end{minipage}%
% }
% \subfigure[]{
%     \begin{minipage}[t]{0.33\linewidth}
%         \centering
%         \includegraphics[width=1.651in]{ADistance.pdf}\\
%         \vspace{0.02cm}
%         %\caption{fig1}
%     \end{minipage}%
% }
% \vspace{-1.5em}
% \end{figure}

% Furthermore, parameter $\alpha$ also plays a crucial role in the proxy of combined risk. It is different from the usage of \textit{mixup} in \cite{zhang2018mixup, berthelot2019mixmatch}, for simplicity, we set $\alpha$ as the fixed value in all the experiments. As shown in Fig. \ref{fig:param}(c), better performance can be achieved when $\alpha$ is set to 0.6. In addition, selecting $\alpha$ in [0.4, 0.6] is recommended.
%1: gamma; 2:alpha; 3:mse and cross-entropy; 4.E-mixup and mixup;

